Quantum Computing

Quantum mechanics---the theory describing the fundamental workings of nature---is famously counterintuitive: it predicts that a particle can be in two places at the same time, and that two remote particles can be inextricably and instantaneously linked. These predictions have been the topic of intense metaphysical debate ever since the theory's inception early last century. However, supreme predictive power combined with direct experimental observation of some of these unusual phenomena leave little doubt as to its fundamental correctness. In fact, without quantum mechanics we could not explain the workings of a laser, nor indeed how a fridge magnet operates. Over the last several decades quantum information science has emerged to seek answers to the question: can we gain some advantage by storing, transmitting and processing information encoded in systems that exhibit these unique quantum properties? Today it is understood that the answer is yes. Many research groups around the world are working towards one of the most ambitious goals humankind has ever embarked upon: a quantum computer that promises to exponentially improve computational power for particular tasks. A number of physical systems, spanning much of modern physics, are being developed for this task---ranging from single particles of light to superconducting circuits---and it is not yet clear which, if any, will ultimately prove successful. Here we describe the latest developments for each of the leading approaches and explain what the major challenges are for the future.

==> ObrienReviewHeader.tex <==
% This is an assortment of those "bare minimum" commands of mine
% needed to compile documents sent to Jeremy.

%GATHER{../common/tex/latex/packages/mycommands.tex}  % Most come from here
\RequirePackage{dcolumn}% Align table columns on decimal point
\RequirePackage{bm}% bold math
\RequirePackage{color}
\RequirePackage{palatino} % makes it look more Nature-ish
\RequirePackage{mathpazo} \RequirePackage{multirow}
\RequirePackage{ifthen}
\newboolean{ispreprint}
\newboolean{versioncontrol}
\setboolean{versioncontrol}{true}

\bibliographystyle{myunsrtnat}

%%%%%%%%%%%%%%%%%%%% small-caps abbreviations.
\newcommand{\abbrev}[1]{{\scshape\lowercase{#1}}}  % see LaTeX Companion, p. 169

% quotations done as macro to switch between American double quotes
% and British single quotes
\newcommand{\qu}[1]{``#1"}

%%%%%%%%%%%%%%%%%%%% Legacy code for et al, latin, etc.
\newcommand\latinfont[1]{\textit{#1}}
\newcommand{\etal}{\latinfont{et al.}}
\newcommand{\bibetal}[2]{{#1 #2 \etal}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% To save typing on all math commands
\newcommand{\mathcommand}[3][0]{\newcommand{#2}[#1]{\ensuremath{#3}}}

\mathcommand[1]{\bra}{\bigl\langle #1\bigr|}
\mathcommand[1]{\ket}{\bigl| #1\bigr\rangle}
\mathcommand[1]{\nth}{#1^{\text{th}}}
\mathcommand\up{\ket\uparrow} \mathcommand\down{\ket\downarrow}

%%% from Chris Monroe
\newcommand{\unit}[1]{\ensuremath{\,\mathrm{#1}}}
\newcommand{\Yb}{\ensuremath{^{171}\mathrm{Yb}^+}}
\newcommand{\state}[4]{\ensuremath{#1\,\,^{#2}\!{#3}_{#4}}}
%\newcommand{\nm}{\unit{nm}}
%\newcommand{\MHz}{\unit{MHz}}
%\newcommand{\ket}[1]{\ensuremath{\left|#1\right\rangle}}
%\newcommand{\up}{\ensuremath{\left|\uparrow\right\rangle}}
%\newcommand{\bra}[1]{\langle{#1}|}
%\newcommand{\down}{\ensuremath{\left|\downarrow\right\rangle}}


\newcommand{\comment}[1]{}

\newcommand{\red}{\textcolor{red}}
\newcommand{\blue}{\textcolor[rgb]{0,0,0.7}}
\newcommand\version[1]{
\ifthenelse{\boolean{versioncontrol}}{
    \vspace{-3ex}\noindent\textit{\red{\small
    #1}}\linebreak[0]}}{}

%%%%%%%%%%%%%%%%%%% Text subscripts
\newcommand{\ts}[2]{\ensuremath{{#1}_{\text{#2}}}}
\newcommand{\tsc}[2]{\ensuremath{{#1}_{\textsc{#2}}}}

%%%%%%%%%%%%%%%%%%% Struts
\newcommand{\mystrut}{\rule{0pt}{2.3ex}}
\newcommand{\tablestrut}{\rule{0ex}{2.6ex}} % Gratzer, p. 151

%%%%%%%%%%%%%%%%%%% frequent symbols/abbreviations
\newcommand{\EJ}{\tsc{E}{j}}
\newcommand{\QC}{\abbrev{QC}}
\newcommand{\NV}{\abbrev{NV}}
\newcommand{\MBE}{\abbrev{MBE}}
\newcommand{\QEC}{\abbrev{QEC}}
\newcommand{\QED}{\abbrev{QED}}
\newcommand{\CQED}{c\abbrev{QED}}
\newcommand{\QND}{\abbrev{QND}}
\newcommand{\NMR}{\abbrev{NMR}}
\newcommand{\CNOT}{controlled-\abbrev{not}}
\newcommand{\RF}{\abbrev{rf}}

%\bibliographystyle{apsrev}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Units
\mathcommand[1]{\power}{\times 10^{#1}}
\mathcommand{\tesla}{\text{~T}}
\mathcommand{\cc}{\text{~cm}^3}
%\mathcommand{\kelvin}{^\circ\text{K}}
\mathcommand{\kelvin}{\text{~K}}
\mathcommand{\percc}{\text{~cm}^{-3}}
\mathcommand{\mol}{\text{~mol}}

\mathcommand{\per}{/\!\!} %Gets rid of that hard space

\renewcommand{\deg}{\ensuremath{^\circ}}

% Energy and Power
\mathcommand{\joule}{\text{~J}}
\mathcommand{\Joule}{\text{~J}}
\mathcommand{\meV}{\text{~meV}}
\mathcommand{\eV}{\text{~eV}}
\mathcommand{\keV}{\text{~keV}}
\mathcommand{\MeV}{\text{~MeV}}
\mathcommand{\GeV}{\text{~GeV}}
\mathcommand{\uW}{\text{~}\mu\text{W}}
\mathcommand{\watts}{\text{~W}}
\mathcommand{\watt}{\watts}
\mathcommand{\volts}{\text{~V}}
% Freq
\mathcommand{\mHz}{\text{~mHz}}
\mathcommand{\Hz}{\text{~Hz}}
\mathcommand{\kHz}{\text{~kHz}}
\mathcommand{\MHz}{\text{~MHz}}
\mathcommand{\GHz}{\text{~GHz}}
\mathcommand{\THz}{\text{~THz}}
\mathcommand{\PHz}{\text{~PHz}}
% Time
\mathcommand{\yr}{\text{~yr}}
\mathcommand{\hr}{\text{~hr}}
\mathcommand{\minutes}{\text{~min}}
\mathcommand{\seconds}{\text{~sec}}
\mathcommand{\second}{\text{~sec}}
%\mathcommand{\sec}{\text{~sec}} Already defined!
\mathcommand{\ms}{\text{~ms}}
\mathcommand{\us}{\text{~}\mu\text{s}}
\mathcommand{\ns}{\text{~ns}}
\mathcommand{\ps}{\text{~ps}}
\mathcommand{\fs}{\text{~ps}}
% Length
\mathcommand{\km}{\text{~km}}
\mathcommand{\meter}{\text{~m}}
\mathcommand{\cm}{\text{~cm}}
\mathcommand{\mm}{\text{~mm}}
\mathcommand{\um}{\text{~}\mu\text{m}}
\mathcommand{\nm}{\text{~nm}}
\mathcommand{\picom}{\text{~pm}}
\mathcommand{\fm}{\text{~fm}}
\mathcommand{\angstr}{\text{~\AA}}
% Mass
\mathcommand{\gram}{\text{~g}}
\mathcommand{\kg}{\text{~kg}}

%%%%%%%%%%%%%%%%%%%%%%%%%%% Constants
\mathcommand{\mub}{\tsc{\mu}{B}}  % Bohr Magneton
\mathcommand{\kb}{\tsc{k}{B}}     % Boltzmann's constant
\mathcommand{\ef}{\tsc{E}{F}}     % The Fermi Energy

